Volumetric Temporal Texture Synthesis for Smoke Stylization using Neural Cellular Automata

Artistic stylization of 3D volumetric smoke data is still a challenge in computer graphics due to the difficulty of ensuring spatiotemporal consistency given a reference style image, and that within reasonable time and computational resources. In this work, we introduce Volumetric Neural Cellular Automata (VNCA), a novel model for efficient volumetric style transfer that synthesizes, in real-time, multi-view consistent stylizing features on the target smoke with temporally coherent transitions between stylized simulation frames. VNCA synthesizes a 3D texture volume with color and density stylization and dynamically aligns this volume with the intricate motion patterns of the smoke simulation under the Eulerian framework. Our approach replaces the explicit fluid advection modeling and the inter-frame smoothing terms with the self-emerging motion of the underlying cellular automaton, thus reducing the training time by over an order of magnitude. Beyond smoke simulations, we demonstrate the versatility of our approach by showcasing its applicability to mesh stylization.

==> sec/table-train.tex <==
\begin{table}

\begin{tabular}{ccccc}
\hline
\small{Methods}  &  SKPN  &  FFTNST  &  \textbf{VNCA}  &  \\
\hline
Training Time   &   76h   &   18h      & 35m \\
Inter-frame Consistency?   & \cmark  & \xmark    & \cmark 
\tabularnewline \hline
\end{tabular}
\caption{\textbf{Training Time Comparison with FFTNST and SKPN.} We reference the paper of \citet{aurand2022efficient} and \citet{guo2021volumetric} for the training time of these methods for a comparison with our measured model training time. FFTNST has no regularization on the temporal consistency of the stylized volume. Our reported training is evaluated on \textit{Billowy} (350$\times$500$\times$350). }
\label{tab:train}
\end{table}
